Uncertainty-driven ensembles of deep architectures for multiclass classification. Application to COVID-19 diagnosis in chest X-ray images

Respiratory diseases kill million of people each year. Diagnosis of these pathologies is a manual, time-consuming process that has inter and intra-observer variability, delaying diagnosis and treatment. The recent COVID-19 pandemic has demonstrated the need of developing systems to automatize the diagnosis of pneumonia, whilst Convolutional Neural Network (CNNs) have proved to be an excellent option for the automatic classification of medical images. However, given the need of providing a confidence classification in this context it is crucial to quantify the reliability of the model's predictions. In this work, we propose a multi-level ensemble classification system based on a Bayesian Deep Learning approach in order to maximize performance while quantifying the uncertainty of each classification decision. This tool combines the information extracted from different architectures by weighting their results according to the uncertainty of their predictions. Performance of the Bayesian network is evaluated in a real scenario where simultaneously differentiating between four different pathologies: control vs bacterial pneumonia vs viral pneumonia vs COVID-19 pneumonia. A three-level decision tree is employed to divide the 4-class classification into three binary classifications, yielding an accuracy of 98.06% and overcoming the results obtained by recent literature. The reduced preprocessing needed for obtaining this high performance, in addition to the information provided about the reliability of the predictions evidence the applicability of the system to be used as an aid for clinicians.

==> elsarticle/biblio.tex <==
@ARTICLE{stivaros,
	author = {S. M. Stivaros and A. Gledson and G. Nenadic and X. J. Zeng and J. Keane and A. Jackson},
	title = {Decision support systems for clinical radiological practice-towards the next generation},
	journal = {British Journal of Radiology},
	year = {2010},
	volume = {83},
	pages = {904-914},
}

@ARTICLE{haxby,
	author = {J. V. Haxby and m. I. Gobbini and M. L. Furey and A. Ishai and J. L. Schouten and P. Pietrini},
	title = {Distributed and overlapping representations of faces and objects in ventral temporal cortex},
	journal = {Science},
	year = {2001},
	volume = {293},
	pages = {2425-2430},
}
